KPI-BERT: A Joint Named Entity Recognition and Relation Extraction Model for Financial Reports

We present KPI-BERT, a system which employs novel methods of named entity recognition (NER) and relation extraction (RE) to extract and link key performance indicators (KPIs), e.g. "revenue" or "interest expenses", of companies from real-world German financial documents. Specifically, we introduce an end-to-end trainable architecture that is based on Bidirectional Encoder Representations from Transformers (BERT) combining a recurrent neural network (RNN) with conditional label masking to sequentially tag entities before it classifies their relations. Our model also introduces a learnable RNN-based pooling mechanism and incorporates domain expert knowledge by explicitly filtering impossible relations. We achieve a substantially higher prediction performance on a new practical dataset of German financial reports, outperforming several strong baselines including a competing state-of-the-art span-based entity tagging approach.

==> figures/prediction-examples.tex <==
% \pgfkeys{%
% /depgraph/reserved/edge style/.style = {%
% -, >=stealth, % arrow properties
% black, solid, line cap=round, % line properties
% rounded corners=2, % make corners round
% },%
% }

% \begin{dependency}[hide label]
% \scriptsize
%     \begin{deptext}
%     In den übrigen \& \color{red}{sonstigen betrieblichen Aufwendungen} \& sind \& Sonstige Steuern \& in Höhe von \& \color{blue}{12,6} \& Mio. \euro{} (im Vorjahr: \& 4,7 \& Mio €) enthalten. \\
%      \& \scriptsize{kpi} \& \& \scriptsize{davon} \& \& \scriptsize{davon-cy} \& \& \scriptsize{davon-py} \& \\
%     \end{deptext}
%     \depedge[edge height=0.2cm]{2}{4}{}
%     \depedge[edge height=0.2cm]{4}{6}{}
%     \depedge[edge height=0.3cm]{4}{8}{}
% \end{dependency}


==> tables/clf_report_ner.tex <==
% \rowcolors{2}{gray!10}{white}
% \begin{tabular}{lcccc}
% \toprule
% in \% &  Precision &  Recall &  F$_1$ &  Support \\
% \midrule
% & $60.57$ & $60.82$ & $60.66$ & \\ \rowcolor{white} \multirow{-2}{*}{kpi}  & \scriptsize ($1.77$)  & \scriptsize ($1.70$)  & \scriptsize ($0.71$) & \multirow{-2}{*}{$486$} \\
% % \multirow{2}{*}{kpi}    &       \makecell[c]{60.57 \\ \scriptsize (1.77)} &    \makecell[c]{60.82 \\ \scriptsize (1.70)} &      \makecell[c]{60.66 \\ \scriptsize (0.71)} &      486 \\
% \rowcolor{gray!10} & $81.65$ & $82.97$ & $82.26$ & \\  \multirow{-2}{*}{cy}  & \scriptsize ($1.68$)  & \scriptsize ($2.40$)  & \scriptsize ($0.89$) & \multirow{-2}{*}{$387$} \\
% % cy             &       \makecell[c]{81.65 \\ \scriptsize (1.68)} &    \makecell[c]{82.97 \\ \scriptsize (2.40)} &      \makecell[c]{82.26 \\ \scriptsize (0.89)} &      387 \\
% & $51.81$ & $54.71$ & $53.19$ & \\ \rowcolor{white} \multirow{-2}{*}{davon}  & \scriptsize ($1.38$)  & \scriptsize ($2.63$)  & \scriptsize ($1.70$) & \multirow{-2}{*}{$208$} \\
% % davon          &       \makecell[c]{51.81 \\ \scriptsize (1.38)} &    \makecell[c]{54.71 \\ \scriptsize (2.63)} &      \makecell[c]{53.19 \\ \scriptsize (1.70)} &      208 \\
% \rowcolor{gray!10} & $73.77$ & $77.43$ & $75.39$ & \\  \multirow{-2}{*}{davon-cy}  & \scriptsize ($4.40$)  & \scriptsize ($3.42$)  & \scriptsize ($1.84$) & \multirow{-2}{*}{$202$} \\
% % davon-cy       &       \makecell[c]{73.77 \\ \scriptsize (4.40)} &    \makecell[c]{77.43 \\ \scriptsize (3.42)} &      \makecell[c]{75.39 \\ \scriptsize (1.84)} &      202 \\
% & $80.74$ & $88.61$ & $84.46$ & \\ \rowcolor{white} \multirow{-2}{*}{py}  & \scriptsize ($1.66$)  & \scriptsize ($1.94$)  & \scriptsize ($0.82$) & \multirow{-2}{*}{$173$} \\
% % py             &       80.74 \scriptsize (1.66) &    88.61 \scriptsize (1.94) &      84.46 \scriptsize (0.82) &      173 \\
% \rowcolor{gray!10} & $81.04$  & $80.35$ & $80.64$ & \\  \multirow{-2}{*}{davon-py}  & \scriptsize ($2.55$)  & \scriptsize ($1.76$)  & \scriptsize ($0.96$) & \multirow{-2}{*}{$114$} \\
% % davon-py       &       81.04 \scriptsize (2.55) &    80.35 \scriptsize (1.76) &      80.64 \scriptsize (0.96) &      114 \\
% & $67.04$ & $48.72$ & $55.94$ & \\ \rowcolor{white} \multirow{-2}{*}{false-positive}  & \scriptsize ($4.81$)  & \scriptsize ($8.73$)  & \scriptsize ($7.27$) & \multirow{-2}{*}{$39$} \\
% % false-positive &       67.04 \scriptsize (4.81) &    48.72 \scriptsize (8.73) &      55.94 \scriptsize (7.27) &       39 \\
% \rowcolor{gray!10} & $58.05$  & $44.62$ & $47.84$ & \\  \multirow{-2}{*}{increase}  & \scriptsize ($15.51$)  & \scriptsize ($14.51$)  & \scriptsize ($8.83$) & \multirow{-2}{*}{$13$} \\
% % increase       &       58.05 \scriptsize (15.51) &    44.62 \scriptsize (14.51) &      47.84 \scriptsize (8.83) &       13 \\
% & $19.77$ & $41.25$ & $26.33$ & \\ \rowcolor{white} \multirow{-2}{*}{kpi-coref}  & \scriptsize ($2.93$)  & \scriptsize ($9.76$)  & \scriptsize ($4.09$) & \multirow{-2}{*}{$8$} \\
% % kpi-coref      &       19.77 \scriptsize (2.93) &    41.25 \scriptsize (9.76) &      26.33 \scriptsize (4.09) &       8 \\
% \rowcolor{gray!10} & $27.07$  & $57.14$ & $36.36$ & \\  \multirow{-2}{*}{decrease}  & \scriptsize ($6.94$)  & \scriptsize ($14.29$)  & \scriptsize ($8.41$) & \multirow{-2}{*}{$7$} \\
% % decrease       &       27.07 \scriptsize (6.94) &    57.14 \scriptsize (14.29) &      36.36 \scriptsize (8.41) &       7 \\
% & $6.31$ & $13.33$ & $8.19$ & \\ \rowcolor{white} \multirow{-2}{*}{attr}  & \scriptsize ($5.12$)  & \scriptsize ($10.00$)  & \scriptsize ($6.01$) & \multirow{-2}{*}{$6$} \\
% % attr           &       6.31 \scriptsize (5.12) &    13.33 \scriptsize (10.00) &      8.19 \scriptsize (6.01) &       6 \\


% % davon-decrease &       0.00 &    0.00 &      0.00 &        1 \\
% % davon-increase &       0.00 &    0.00 &      0.00 &        1 \\
% % decrease-py    &       - &    - &      - &        0 \\
% % increase-py    &       - &    - &      - &        0 \\
% % py1            &       - &    - &      - &        0 \\
% \midrule
% % ADJUST VALUES
% & $68.39$  & $70.89$ & $69.61$ & \\ \rowcolor{white} \multirow{-2}{*}{micro avg}  & \scriptsize ($0.94$)  & \scriptsize ($0.38$)  & \scriptsize ($0.53$) & \multirow{-2}{*}{$1643$} \\
% % \rowcolor{white} micro avg      &       68.39 \scriptsize (0.94) &    70.80 \scriptsize (0.38) &      69.57 \scriptsize (0.52) &     1645 \\
% & $55.26$ & $59.09$ & $55.57$ & \\ \rowcolor{white} \multirow{-2}{*}{macro avg}  & \scriptsize ($1.44$)  & \scriptsize ($1.71$)  & \scriptsize ($1.19$) & \multirow{-2}{*}{$1643$} \\
% % macro avg      &       46.75 \scriptsize (1.22) &    50.00 \scriptsize (1.44) &      47.02 \scriptsize (1.00) &     1645 \\
% % \rowcolor{white} weighted avg      &       68.39 \scriptsize (0.94) &    70.80 \scriptsize (0.38) &      69.57 \scriptsize (0.52) &     1645 \\
% \bottomrule
% \end{tabular}
% 
% 
% \rowcolors{2}{gray!10}{white}
% \begin{tabular}{lcccc}
% \toprule
% in \% &  Precision &  Recall &  F$_1$ &  Support \\
% \midrule
% kpi & $60.57$ \scriptsize ($1.77$) & $60.82$ \scriptsize ($1.70$) & $60.66$ \scriptsize ($0.71$) & $486$ \\ 
% cy  & $81.65$ \scriptsize ($1.68$) & $82.97$ \scriptsize ($2.40$) & $82.26$ \scriptsize ($0.89$) & $387$ \\ 
% davon & $51.81$ \scriptsize ($1.38$) & $54.71$ \scriptsize ($2.63$) & $53.19$ \scriptsize ($1.70$) & $208$ \\ 
% davon-cy  & $73.77$ \scriptsize ($4.40$) & $77.43$ \scriptsize ($3.42$) & $75.39$ \scriptsize ($1.84$) & $202$ \\  
% py & $80.74$ \scriptsize ($1.66$) & $88.61$ \scriptsize ($1.94$) & $84.46$ \scriptsize ($0.82$) & $173$ \\ 
% davon-py  & $81.04$  \scriptsize ($2.55$) & $80.35$ \scriptsize ($1.76$) & $80.64$ \scriptsize ($0.96$) & $114$ \\  
% false-positive & $67.04$ \scriptsize ($4.81$) & $48.72$ \scriptsize ($8.73$) & $55.94$ \scriptsize ($7.27$) & $39$ \\ 
% increase  & $58.05$  \scriptsize ($15.51$) & $44.62$ \scriptsize ($14.51$) & $47.84$ \scriptsize ($8.83$) & $13$ \\  
% kpi-coref & $19.77$ \scriptsize ($2.93$) & $41.25$ \scriptsize ($9.76$) & $26.33$ \scriptsize ($4.09$) & $8$ \\ 
% decrease  & $27.07$  \scriptsize ($6.94$) & $57.14$ \scriptsize ($14.29$) & $36.36$ \scriptsize ($8.41$) & $7$ \\  
% attr & $6.31$ \scriptsize ($5.12$) & $13.33$ \scriptsize ($10.00$) & $8.19$ \scriptsize ($6.01$) & $6$ \\ 


% % davon-decrease &       0.00 &    0.00 &      0.00 &        1 \\
% % davon-increase &       0.00 &    0.00 &      0.00 &        1 \\
% % decrease-py    &       - &    - &      - &        0 \\
% % increase-py    &       - &    - &      - &        0 \\
% % py1            &       - &    - &      - &        0 \\
% \midrule
% % ADJUST VALUES
% % & $68.39$  & $70.89$ & $69.61$ & \\ \rowcolor{white} \multirow{-2}{*}{micro avg}  & \scriptsize ($0.94$)  & \scriptsize ($0.38$)  & \scriptsize ($0.53$) & \multirow{-2}{*}{$1643$} \\
% \rowcolor{white} micro avg      &       $68.39$ \scriptsize ($0.94$) &    $70.89$ \scriptsize ($0.38$) &      $69.61$ \scriptsize ($0.53$) &     $1643$ \\
% % & $55.26$ & $59.09$ & $55.57$ & \\ \rowcolor{white} \multirow{-2}{*}{macro avg}  & \scriptsize ($1.44$)  & \scriptsize ($1.71$)  & \scriptsize ($1.19$) & \multirow{-2}{*}{$1643$} \\
% macro avg      &       $55.26$ \scriptsize ($1.44$) &    $59.09$ \scriptsize ($1.71$) &      $55.57$ \scriptsize ($1.19$) &     $1643$ \\
% % \rowcolor{white} weighted avg      &       68.39 \scriptsize (0.94) &    70.80 \scriptsize (0.38) &      69.57 \scriptsize (0.52) &     1645 \\
% \bottomrule
% \end{tabular}
%
%
%
\scriptsize
\rowcolors{2}{gray!10}{white}
% \addtolength{\tabcolsep}{3\tabcolsep}
\sisetup{input-symbols = {()}}  % , table-space-text-post = ), table-space-text-pre = (
\begin{tabular}{l@{\hspace{\tabcolsep}}S@{\hspace{\tabcolsep}}SS@{\hspace{\tabcolsep}}SS@{\hspace{\tabcolsep}}S@{\hspace{\tabcolsep}}S[table-format = 4]}  % @{\hspace{2\tabcolsep}}
% \begin{tabular}{lSSSSSSS[table-format = 4]} 
\toprule
in \% &  \multicolumn{2}{c}{Precision} &  \multicolumn{2}{c}{Recall} &  \multicolumn{2}{c}{F$_1$} &  Support \\
\midrule
kpi & 76.76 & (0.73) & 78.66 & (0.61) & 77.69 & (0.57) & 796 \\ 
cy  & 86.98 & (1.05) & 86.75 & (1.39) & 86.86 & (0.79) & 560 \\ 
davon & 67.54 & (0.99) & 71.93 & 0.94) & 69.66 & (0.56) & 419 \\ 
davon-cy  & 80.22 & (1.43) & 85.81 & (1.09) & 82.91 & (0.71) & 401 \\  
py & 90.83 & (1.49) & 88.57 & (1.44) & 89.67 & (0.91) & 272 \\ 
davon-py  & 86.13  & (1.60) & 91.89 & (1.94) & 88.89 & (1.04) & 233 \\  
% false-positive & 67.04 & (4.81) & 48.72 & (8.73) & 55.94 & (7.27) & 39 \\ 
increase  & 63.57  & (5.52) & 62.35 & (6.55) & 62.50 & (3.36) & 17 \\  
% kpi-coref & 19.77 & (2.93) & 41.25 & (9.76) & 26.33 & (4.09) & 8 \\ 
decrease  & 57.21  & (9.37) & 55.00 & (11.46) & 55.02 & (7.31) & 8 \\  
% attr & 6.31 & (5.12) & 13.33 & (10.00) & 8.19 & (6.01) & 6 \\ 

\midrule
% ADJUST VALUES
% & 68.39  & 70.89 & 69.61 & \\ \rowcolor{white} \multirow{-2}{*}{micro avg}  & \scriptsize (0.94)  & \scriptsize (0.38)  & \scriptsize (0.53) & \multirow{-2}{*}{1643} \\
\rowcolor{white} micro avg      &       79.88 & (0.55) &    82.31 & (0.53) &      81.08 & (0.53) &     2706 \\
% & 55.26 & 59.09 & 55.57 & \\ \rowcolor{white} \multirow{-2}{*}{macro avg}  & \scriptsize (1.44)  & \scriptsize (1.71)  & \scriptsize (1.19) & \multirow{-2}{*}{1643} \\
macro avg      &       76.16 & (0.99) &    77.62 & (1.51) &      76.65 & (1.10) &     2706 \\
% \rowcolor{white} weighted avg      &       68.39 \scriptsize (0.94) &    70.80 \scriptsize (0.38) &      69.57 \scriptsize (0.52) &     1645 \\
\bottomrule
\end{tabular}
% \addtolength{\tabcolsep}{-3\tabcolsep}

==> tables/prediction_examples_translated.tex <==
\begin{tabularx}{\linewidth}{lXr}
\toprule
& Sentence with predicted Entities & Relations \\
\midrule
(a) & Correct relation predictions and annotations. & \\
\midrule
1 & The {\color{ForestGreen}{[$\underset{\text{kpi}}{\text{other assets}}$}]} include ``{\color{ForestGreen}{[$\underset{\text{davon}}{\text{earmarked loans}}$}]}'' amounting to TEUR {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{25}}$}]} (prior year: TEUR {\color{ForestGreen}{[$\underset{\text{davon-py}}{\text{25}}$}]}), which were given to franchise partners in fiscal year 2004 to 2007.  & 
\tiny{\color{ForestGreen}{\makecell[r]{kpi -- davon\\ 
davon -- davon-cy \\
davon -- davon-py}}} \\
% still correct
\midrule
2 & The {\color{ForestGreen}{[$\underset{\text{attr}}{\text{members of the supervisory board }}$}]} received T\euro{} {\color{ForestGreen}{[$\underset{\text{cy}}{\text{368}}$}]} (prior year T\euro{}  {\color{ForestGreen}{[$\underset{\text{py}}{\text{242}}$}]}) as  {\color{ForestGreen}{[$\underset{\text{kpi}}{\text{total compensation}}$}]} in fiscal year 2007. & 
\tiny{\color{ForestGreen}{\makecell[r]{kpi -- attr\\
kpi -- cy \\
kpi -- py}}} \\

%Die Mitglieder des Aufsichtsrates haben im Geschäftsjahr 2007 eine Gesamtvergütung in Höhe von T € 368 ( Vj . T € 368 ) erhalten .
% still correct
\midrule
(b) & Minor differences between ground truth annotations and model predictions. Arguably, the model predictions are correct, but an annotation mismatch leads to a sentence F$_1$-score below 1. & \\
\midrule
3 & {\color{NavyBlue}{[Raw,}} {\color{Red}{[$\underset{\text{{\color{NavyBlue}{kpi}} kpi}}{\text{auxiliary and operating materials}}$}]}{\color{NavyBlue}{]}} in the amount of {\color{ForestGreen}{[$\underset{\text{cy}}{\text{56,9}}$}]} M. \euro{} (prior year {\color{ForestGreen}{[$\underset{\text{py}}{\text{50,3}}$}]} M. \euro{}) are mainly allocated to medical requirements. & 
\tiny{\color{NavyBlue}{\makecell[r]{kpi -- cy\\
kpi -- py \\
\color{Red}{kpi -- cy} \\ 
\color{Red}{kpi -- py}}}} \\

% 3 & In den {\color{ForestGreen}{[$\underset{\text{kpi}}{\text{Löhnen und Gehältern}}$}]} werden in Höhe von {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{2,4}}$}]} Mio. \euro{} (im Vorjahr: {\color{ForestGreen}{[$\underset{\text{davon-py}}{\text{2,1}}$}]} Mio. \euro{}) {\color{Red}{[für}} {\color{NavyBlue}{[$\underset{\text{{\color{Red}{davon}} davon}}{\text{Mitarbeiter übernommene Lohn- und Kirchensteuer}}$}]}{\color{Red}{]}} ausgewiesen. & 
% \tiny{\color{NavyBlue}{\makecell[r]{kpi -- davon\\
% davon -- davon-cy \\
% davon -- davon-py \\ 
% \color{Red}{kpi -- davon} \\ 
% \color{Red}{davon -- davon-cy} \\
% \color{Red}{davon -- davon-py}}}} \\

% Roh - , Hilfs - und Betriebsstoffe in Höhe von 56,9 Mio . € ( Vj . 50,3 Mio . €) betreffen im Wesentlichen den medizinischen Bedarf .

% still correct

\midrule
4 & In 2011, {\color{Red}{[the }} {\color{NavyBlue}{[$\underset{\text{{\color{Red}{kpi}} kpi}}{\text{performance-related share}}$}]}{\color{Red}{]}} is composed of  {\color{ForestGreen}{[$\underset{\text{davon}}{\text{short term components}}$}]} in the amount of TEUR {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{150}}$}]} (corresponding to 75\% of the performance-related share), which will be paid off during the following fiscal year, and  {\color{ForestGreen}{[$\underset{\text{davon}}{\text{long term components}}$}]} in the amount of TEUR {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{48}}$}]} (corresponding to 25\% of the performance-related share). & 
\tiny{\color{Red}{\makecell[r]{kpi -- davon\\
kpi -- davon \\
\color{NavyBlue}{kpi -- davon} \\
\color{NavyBlue}{kpi -- davon} \\
\color{ForestGreen}{davon -- davon-cy} \\ 
\color{ForestGreen}{davon -- davon-cy}}}} \\

% Der erfolgsbezogene Anteil 2011 setzt sich aus der kurzfristigen Komponente in Höhe von TEUR 150 ( entspricht 75 % des erfolgsbezogenen Anteils ) , die innerhalb eines folgenden Geschäftsjahres ausgezahlt wird , und der langfristigen Komponente in Höhe von TEUR 48 ( entspricht 25 % des erfolgsbezogenen Anteils ) zusammen .
\midrule
(c) & Wrong ground truth annotations, but arguably correct model predictions. & \\
\midrule
5 & {\color{NavyBlue}{[$\underset{\text{kpi-coref}}{\text{These}}$}]} include {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon \color{Red}{kpi}}}{\text{revenues from not yet billed service contracts]}}$}}{\color{Red}{]}} in the amount of T\euro{}  {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-cy \color{Red}{cy}}}{\text{6.848}}$}]}{\color{Red}{]}} (prior year T\euro{} {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-py \color{Red}{py}}}{\text{3.950}}$}]}{\color{Red}{]}}), which are realised in accordance to the stage of completion.  & 
\tiny{\color{NavyBlue}{\makecell[r]{kpi-coref -- davon\\
davon -- davon-cy \\
davon -- davon-py \\
{\color{Red}{kpi -- cy}} \\
{\color{Red}{kpi -- py}}}}} \\

% Sie beinhalten Erlöse aus noch nicht abgerechneten Dienstleistungsaufträgen in Höhe von T € 6.848 ( Vj . T € 3.950 ) , die nach dem Leistungsfortschritt realisiert wurden .
\midrule
% 6 & Die {\color{NavyBlue}{[$\underset{\text{kpi}}{\text{Bezüge}}$}]} der im Geschäftsjahr {\color{NavyBlue}{[aktiven}} {\color{Red}{[$\underset{\text{{\color{NavyBlue}{attr}} kpi}}{\text{Geschäftsführungsmitglieder}}$}]}{\color{NavyBlue}{]}} (nur die Bezüge, die an die TC Touristik für entsprechende Tätigkeiten weiterbelastet wurden) belaufen sich für das Jahr 2009/10 auf TEUR {\color{ForestGreen}{[$\underset{\text{cy}}{\text{1.559}}$}]}. & 

% 6 & The {\color{ForestGreen}{[$\underset{\text{kpi}}{\text{interest expenses}}$}]} include TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-cy \color{Red}{cy}}}{\text{848}}$}]}{\color{Red}{]}} (prior year TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-py \color{Red}{py}}}{\text{816}}$}]}{\color{Red}{]}}) for the {\color{NavyBlue}{[$\underset{\text{davon}}{\text{compounding of long term accruals}}$}]}, in particular for retirements, partial retirements and anniversaries and TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-cy \color{Red}{cy}}}{\text{317}}$}]}{\color{Red}{]}} (prior year TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-py \color{Red}{py}}}{\text{432}}$}]}{\color{Red}{]}}) for  {\color{NavyBlue}{[$\underset{\text{davon}}{\text{remunerations of factoring services}}$}]}.
6 & The {\color{ForestGreen}{[$\underset{\text{kpi}}{\text{interest expenses}}$}]} include TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-cy \color{Red}{cy}}}{\text{848}}$}]}{\color{Red}{]}} (prior year TEUR {\color{Red}{[}}{\color{NavyBlue}{[$\underset{\text{davon-py \color{Red}{py}}}{\text{816}}$}]}{\color{Red}{]}}) for the {\color{NavyBlue}{[$\underset{\text{davon}}{\text{compounding of long term accruals}}$}]}, in particular for retirements, partial retirements and anniversaries and TEUR {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{317}}$}]} (prior year TEUR {\color{ForestGreen}{[$\underset{\text{davon-cy}}{\text{432}}$}]}) 
{\color{NavyBlue}{[for}}
{\color{Red}{[$\underset{\text{\color{NavyBlue}{davon} \color{Red}{davon}}}{\text{remunerations of factoring services]}}$}}{\color{NavyBlue}{]}}.
&
\tiny{\makecell[r]{
\color{NavyBlue}{kpi -- davon} \\ 
\color{NavyBlue}{kpi -- davon} \\ 
\color{NavyBlue}{davon-cy -- davon} \\ 
\color{NavyBlue}{davon-py -- davon} \\ 
\color{NavyBlue}{davon-cy -- davon} \\ 
\color{NavyBlue}{davon-py -- davon} \\ 
\color{Red}{kpi -- cy} \\
\color{Red}{kpi -- py} \\
\color{Red}{kpi -- cy} \\
\color{Red}{kpi -- py}}} \\

% In den Zinsaufwendungen sind TEUR 848 ( VJ TEUR 816 ) für die Aufzinsung von langfristigen Rückstellungen , insbesondere für Pensionen , Altersteilzeit und Jubiläum und TEUR 327 ( VJ TEUR 432 ) Entgelte für Factoring-Geschäfte enthalten .

\bottomrule
\end{tabularx}

